Explaining Realized Returns: Roll's $R^2$ 40 Years Later

Can we explain asset price movements even with hindsight? Reinterpreting Roll's (1988) AFA Presidential Address, "$R^2$," as a modern empirical exercise, we show that conventional macroeconomic, cash-flow, expectations, and flow variables explain less than 10% (often with negative $R^2$) of monthly U.S. equity return variation out of sample and lack daily observations. We use generative AI to extract reasons stated in Wall Street Journal market summaries while filtering out price-related language. These reasons explain around 30-40% of daily and monthly return variation out of sample. Their content spans interpretable themes, including corporate news, macroeconomic conditions, monetary policy, sentiment, and geopolitics.

==> tables/prompts/flag_reason.tex <==
Please process a list of news excerpts used to analyze their impact on financial markets. The goal is to flag whether a statement contains direct information about a financial asset's price fluctuation during the day.

For example,
Stock market indices (e.g., Nasdaq, S&P 500, or general terms like "US stocks", "most indexes")
Individual stock or sector price changes (e.g., "tech stocks", "bonds")
Treasury bond price or yield changes
Currencies and commodities (e.g., gold, oil, and even cryptocurrencies).

Be vigilant to detect any information on asset price, including subtle language like "pulled back", "rebounded", "buoyed", "hit record".
Flag it with the name of the asset and one or two words for the price action, using the exact same words from the input text.

Otherwise, if there is certainly no such asset price information, flag it with "ok". Note: It is "ok" as long as the information is not about financial market prices. For example, statements about interest rates, firm fundamental, government policy, and the economy should be flagged as "ok".

Output must be in JSON format. Example:
{
	"Oil pushed above $40 a barrel for the first time since June 1": "Oil: xxx",
	"General Motors announced a $15.5 billion second-quarter loss": "ok"
}

==> tables/prompts/movement_reason_prompt.tex <==
You are an expert financial analyst. Please use your understanding of how financial asset prices respond to news, carefully parse this news article, which reports all kinds of recent asset market price movements with reasons and explanations to the observed price changes. Your job is to identify price movement and reason statements and extract them in a structured format. 
If a sentence includes both a price movement and its reason, distinguish them separately.

Output a JSON list of items with "reason" and "price_movement" keys:

IMPORTANT: ONLY USE DIRECT QUOTES FROM THE NEWS ARTICLE.

For example input:
...U.S. stocks slid while crude prices extended recent gains after the European Union said it would impose an oil embargo on Russia...

Report the following item in the JSON list:
{
	"reason": "the European Union said it would impose an oil embargo on Russia",
	<EXPLANATION: reason excerpt should include world events, economic and corporate news, investor sentiment, or other factors that are explicitly stated as causing the observed market price movements. Notice, the reason excerpt should NOT be about the financial market price.>
	"price_movement": "crude prices extended recent gains"
	<EXPLANATION: price movement excerpt should be solely about the price movement. The subject must be an asset/security price or price index; the action is, e.g. price went up or down; also include the time period if mentioned. The reason and price movement should contain the exact wordings in the article, and they should not overlap.>
}

==> tables/prompts/reason_gpt_predict_prompt_display.tex <==
You are an expert financial analyst specializing in the U.S. stock market's response to news events. Your task is to carefully analyze the given sentences, assess their implications for market returns, and predict the potential impact on the overall stock market.
1. Quantifying the potential contribution to stock market return in percentage.
2. Evaluating the surprise level of the event, noting that highly anticipated events typically cause smaller price changes.
3. Assessing the clarity of the event's impact on stock prices, addressing ambiguous effects when both positive and negative forces are present.
4. Delivering an overall evaluation of the expected market return impact in percentage.
Your analysis must integrate economic principles, historical trends, and key financial concepts. Use clear, professional, and neutral language to deliver actionable insights. Simplify complex ideas when needed to suit varying levels of financial literacy while maintaining accuracy and context-specific relevance.
When multiple reasons/events are provided for the same day, you will analyze each one individually first, then aggregate these individual analyses and provide a final overall evaluation in return in percentage decimal without percentage sign, reflecting how much the stock market can be moved due to the combined impact of the provided events.
Strictly return the result in the following JSON format:
```json
{
"result": float number, predicted total market change in percentage decimal without the percentage sign,
"analysis": string, general analysis of the sentences, focusing on the factors above
}
```

